Trust, but Verify: Cross-Modality Fusion for HD Map Change Detection

High-definition (HD) map change detection is the task of determining when sensor data and map data are no longer in agreement with one another due to real-world changes. We collect the first dataset for the task, which we entitle the Trust, but Verify (TbV) dataset, by mining thousands of hours of data from over 9 months of autonomous vehicle fleet operations. We present learning-based formulations for solving the problem in the bird's eye view and ego-view. Because real map changes are infrequent and vector maps are easy to synthetically manipulate, we lean on simulated data to train our model. Perhaps surprisingly, we show that such models can generalize to real world distributions. The dataset, consisting of maps and logs collected in six North American cities, is one of the largest AV datasets to date with more than 7.8 million images. We make the data available to the public at https://www.argoverse.org/av2.html#mapchange-link, along with code and models at https://github.com/johnwlambert/tbv under the the CC BY-NC-SA 4.0 license.

==> latex/tex/TODO.tex <==

% stuff papers

% coco-stuff
% D. Forsyth, J. Malik, M. Fleck, H. Greenspan, T. Leung,
% S. Belongie, and C. Bregler. Finding pictures of objects in
% large collections of images. In International Workshop on
% Object Representation in Computer Vision, 1996.


%  J. Xiao, J. Hays, K. Ehinger, A. Oliva, and A. Torralba. SUN
% database: Large-scale scene recognition from Abbey to Zoo.
% In CVPR, 2010.

% A. Ion, J. Carreira, and C. Sminchisescu. Probabilistic joint
% image segmentation and labeling. In NIPS, pages 1827–
% 1835, 2011.

% J. Tighe and S. Lazebnik. Finding things: Image parsing with
% regions and per-exemplar detectors. In CVPR, 2013.

% J. R. R. Uijlings, K. E. A. van de Sande, T. Gevers, and
% A. W. M. Smeulders. Selective search for object recognition.
% IJCV, 2013.

% R. Mottaghi, S. Fidler, J. Yao, R. Urtasun, and D. Parikh. Analyzing semantic segmentation using hybrid human-machine
% CRFs. In CVPR, pages 3143–3150, 2013

% I. Endres and D. Hoiem. Category-independent object
% proposals with diverse ranking. IEEE Trans. on PAMI,
% 36(2):222–234, 2014.

% J. Dai, K. He, and J. Sun. Convolutional feature masking for
% joint object and stuff segmentation. In CVPR, 2015.

% J. Tighe, M. Niethammer, and S. Lazebnik. Scene parsing with object instances and occlusion ordering. In CVPR,
% 2014

% B. Kim, M. Sun, P. Kohli, and S. Savarese. Relating things
% and stuff by high-order potential modeling. In ECCV, 2012.




% https://openaccess.thecvf.com/content_ECCVW_2018/papers/11130/Varghese_ChangeNet_A_Deep_Learning_Architecture_for_Visual_Change_Detection_ECCVW_2018_paper.pdf
% ChangeNet: A Deep Learning Architecture for Visual Change Detection


% Change Detection in High Resolution Satellite Images Using an Ensemble of Convolutional Neural Networks
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8659603&casa_token=gvYW78hsdqEAAAAA:zVuQJR-e4wSWJAleWM5n7Pgo8k3Q8abTrNP2i5N9H8LGI3sFGzZ2NEziXPlKkswV0x-h_u_e&tag=1

% Learning to Measure Changes: Fully Convolutional Siamese Metric Networks for Scene Change Detection
% https://arxiv.org/pdf/1810.09111.pdf

% https://arxiv.org/pdf/1703.00552.pdf
% Change Detection under Global Viewpoint Uncertainty

% Procedural Synthesis of Remote Sensing Images for Robust Change Detection with Neural Networks
% https://arxiv.org/pdf/1905.07877.pdf

% https://openaccess.thecvf.com/content_CVPR_2019/papers/Revaud_Did_It_Change_Learning_to_Detect_Point-Of-Interest_Changes_for_Proactive_CVPR_2019_paper.pdf
% Did it change? Learning to Detect Point-of-Interest Changes for Proactive Map Updates

% https://dl.acm.org/doi/pdf/10.1145/3356471.3365232?casa_token=SpwGrukU4gQAAAAA%3Aa2qVTHcpCYBdBfUpxtLQ7xdAvtwe_mbf0mm5oThf-jdd4YEHLHSUNqLBmVXFWGU9TrF3QQIaxvgn
% ChangeNet: Learning to Detect Changes in Satellite Images

% Self-supervised Simultaneous Alignment and Change Detection
% http://ras.papercept.net/images/temp/IROS/files/1888.pdf

% Efficient GAN-Based Remote Sensing Image Change Detection Under Noise Conditions
% https://link.springer.com/chapter/10.1007/978-3-030-51859-2_1

% https://www.ri.cmu.edu/wp-content/uploads/2019/06/Christensen_Masters_Thesis_Final.pdf

% https://ieeexplore.ieee.org/document/8794329/

% https://www.hindawi.com/journals/mpe/2015/713753/

% Road image update using in-vehicle camera images and aerial image

% A New Approach to High-accuracy Road Orthophoto Mapping Based on Wavelet Transform http://ir.nsfc.gov.cn/paperDownload/1000003472018.pdf
% Generation and Exploitation of Local Orthographic  Imagery for Road Vehicle Localisation. Ashley Napier and Paul Newman.
%

% https://www.researchgate.net/publication/327737058_Simultaneous_Localization_and_Map_Change_Update_for_the_High_Definition_Map-Based_Autonomous_Driving_Car



==> neurips-21/neurips-checklist.tex <==





\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} % see Abstract.}
  \item Did you describe the limitations of your work?
   \answerYes{See `Limitations' in Section~\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We blur identifiable information. See Datasheet in the Supplementary Material.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Ethical considerations include dataset accessibility  and privacy (See Datasheet in the Supplementary Material).}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Data is shared with the reviewers. Code is public at \url{https://github.com/johnwlambert/tbv}. Section \ref{sec:impldetails} describes experimental protocols.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:impldetails}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Performance varies little with random restarts and there is considerable computational cost for training redundant models.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see the Supplementary Material. }
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{ } % Our dataset does not use existing assets, but our development kit does draw on existing 3rd party libraries such as Numpy, Open3d, and OpenCV.
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The dataset is provided to reviewers through a private url.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
     \answerYes{See Supplemental Data Sheet.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Supplemental Data Sheet. All identifiable data is blurred.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{Neither crowdsourcing nor research on human subjects was used.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
